LHC data and its impact on nCTEQ15 PDFs

The LHC heavy ion data for W/Z production can provide new incisive information on the PDFs. This data is sensitive to the heavier quark flavors (strange and charm) in a high energy kinematic region; this can facilitate the determination of PDFs in the small x region where previous data was limited. At present, the flavor separation of the proton PDFs is dependent on DIS data from nuclear targets. Therefore, improved nuclear corrections can also yield enhanced flavor determination of both the proton and nuclear PDFs.

==> figdef.tex <==


\def\figone{
\begin{figure}[th] %%%%%%%%%%%%%%%%%%%%%
\centering{} 
\includegraphics[width=0.48\textwidth]{figs/F2AF2Dcompare_F2_0_56_26_5.pdf}
\hfill
\includegraphics[width=0.48\textwidth]{figs/F2AF2Dcompare_F2_1_56_26_5.pdf}
\caption{Predictions from Ref.~\cite{Kovarik:2010uv}  for the nuclear correction factors ($A=Fe$) with
(a) $R[F_{2}^{\ell A}]\simeq F_{2}^{\ell A}/F_{2}^{\ell N}$ 
and (b) $R[F_{2}^{\nu A}]\simeq F_{2}^{\nu A}/F_{2}^{\nu N}$  
as a function of $x$ for $Q^{2}=5\,{\rm GeV}^{2}$. The data points
displayed in (a) are from BCDMS and SLAC experiments
and those displayed in (b) come from the NuTeV experiment.
}
\label{fig:one}
\end{figure} %%%%%%%%%%%%%%%%%%%%%%%%
}




\def\figtwo{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
\begin{subfigure}[t]{0.55\textwidth} %%%%%%%%%%%%%%%%%%%%%
\centering{} 
\includegraphics[width=0.95\textwidth]{figs/strange.pdf}
\caption{The strange PDF at $Q=3$~GeV vs.\ $x$ for the set of PDFs 
displayed in Fig.~\ref{fig:one}.
The solid lines show the  central values, 
and the span of the curves provides a measure of the nuclear PDF uncertainty. 
}
\label{fig:twoa}
\end{subfigure} %%%%%%%%%%%%%%%%%%%%%%%%
%
\hfill
%
\begin{subfigure}[t]{0.40\textwidth} %%%%%%%%%%%%%%%%%%%%%
\centering{} 
\includegraphics[width=0.95\textwidth]{figs/spdf.pdf}
\caption{The scaled cross section $d\sigma/dy$ for $W^+$ production at 
the LHC ($\sqrt{s}$=13~TeV). 
The upper (red) curve is the total with uncertainties. 
and the lower curves are (in order) the 
 $u\bar{d}$~(green), $c\bar{s}$~(magenta), $u\bar{s}$~(blue), $c\bar{d}$~(cyan) contributions. 
}
\label{fig:twob}
\end{subfigure} %%%%%%%%%%%%%%%%%%%%%%%%
%
\caption{\null}
\label{fig:two}
\end{figure} %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}



\def\figncteq{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t] %%%%%%%%%%%%%%%%%%%%%
\centering{} 
\includegraphics[width=0.99\textwidth]{figs/nCTEQ15_gs.pdf}
\caption{Selected nCTEQ15 PDFs (gluon, strange) vs.\ $x$ at  $Q=10$~GeV 
for a proton in a lead nucleus, $f^{p/Pb}(x,Q)$. 
We display the central values (solid line) and the uncertainty band  (shaded region)
for 
nCTEQ15\cite{Kovarik:2015cma},
HKN07\cite{Hirai:2007sx},
EPS09\cite{Eskola:2009uj}
and
DSSZ\cite{deFlorian:2011fp}.
}
\label{fig:ncteq15}
\end{figure} %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}


\def\figfour{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
\includegraphics[width=0.75\textwidth]{figs/structRatiosLog.pdf}
\caption{The nuclear correction factors $F_2^A/F_2^N$ for the nCTEQ15\cite{Kovarik:2015cma}
PDFs with uncertainty bands. 
}
\label{fig:four}
\end{figure} %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}





\def\figfive{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
%
\includegraphics[width=0.60\textwidth]{figs/correlation_xsec_Wp_Wm_1F_vs_all.pdf}
\caption{
Preliminary results for the comparison of $W^\pm$ cross section
correlations for only one family $(u,d)$ of
quarks (circles) and all families (triangles) in proton-lead collisions.\cite{newpaper}
% We show here results for nCTEQ15, EPS+CT10, EPS+CTEQ6.1 and CT10 PDFs.
}
\label{fig:five}
\end{figure} %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}



